Performance Modeling for Dense Linear Algebra

It is well known that the behavior of dense linear algebra algorithms is greatly influenced by factors like target architecture, underlying libraries and even problem size; because of this, the accurate prediction of their performance is a real challenge. In this article, we are not interested in creating accurate models for a given algorithm, but in correctly ranking a set of equivalent algorithms according to their performance. Aware of the hierarchical structure of dense linear algebra routines, we approach the problem by developing a framework for the automatic generation of statistical performance models for BLAS and LAPACK libraries. This allows us to obtain predictions through evaluating and combining such models. We demonstrate that our approach is successful in both single- and multi-core environments, not only in the ranking of algorithms but also in tuning their parameters.

==> Makefile <==
PDFLATEX = pdflatex -shell-escape

TARGET = main.pdf

TEXFILES = *.tex figures/*.tex

once: 
	time $(PDFLATEX) main

twice:
	make once
	make once

figs:
	time make -j 4 -B -f main.makefile

bib:
	bibtex main

all:
	make once
	make figs
	make bib
	make once
	make figs
	make twice

bg:
	make once < /dev/null 2>&1 1> /dev/null &

figtest:
	$(PDFLATEX) figtest
	#time make -j 2 -B -f figtest.makefile
	#$(PDFLATEX) figtest.tex

title:
	$(PDFLATEX) title

check: $(TEXFILES)
	for file in $(TEXFILES); \
	do \
		aspell --lang=EN --mode=tex check $$file; \
	done

clean:
	rm -rf main.{aux,log,toc,pdf,lof,out,figlist,makefile,pyg} figures/externalized/*

